COVID-19 Tests Gone Rogue: Privacy, Efficacy, Mismanagement and Misunderstandings

COVID-19 testing, the cornerstone for effective screening and identification of COVID-19 cases, remains paramount as an intervention tool to curb the spread of COVID-19 both at local and national levels. However, the speed at which the pandemic struck and the response was rolled out, the widespread impact on healthcare infrastructure, the lack of sufficient preparation within the public health system, and the complexity of the crisis led to utter confusion among test-takers. Invasion of privacy remains a crucial concern. The user experience of test takers remains low. User friction affects user behavior and discourages participation in testing programs. Test efficacy has been overstated. Test results are poorly understood resulting in inappropriate follow-up recommendations. Herein, we review the current landscape of COVID-19 testing, identify four key challenges, and discuss the consequences of the failure to address these challenges. The current infrastructure around testing and information propagation is highly privacy-invasive and does not leverage scalable digital components. In this work, we discuss challenges complicating the existing covid-19 testing ecosystem and highlight the need to improve the testing experience for the user and reduce privacy invasions. Digital tools will play a critical role in resolving these challenges.

==> content/solutions.tex <==
\section{Solutions, Technological Tools, and their Unintended Consequences}

Overcoming the privacy, test efficacy, workflow, and communication challenges outlined here demands a transformative change. Technological tools designed to address these challenges and mitigate the resulting consequences provide an opportunity to stop the COVID-19 pandemic.  Digital tools are of particular importance in ending the COVID-19 pandemic due to the complexity and interwoven nature of these challenges. 

So advances in probabilistic matching techniques and tools like record linkage helped solve the problem concerning changing data formats and missing data but they compare individual attributes where the algorithm is not aware of the amount of importance that has to be given to individual features to estimate holistically about the potential matches.


\textbf{Improving communication of test results. }Providing a‘ time window’ of what test results mean and how long that info is valid, Improving the performance and relevancy of dependence on an antibody test, Establishment of Online Marketplaces, Increase in the number of tests, Addressing User Trust Issues, Precautionary measures to cope with glitches in testing results. It is important to check the spread of rumors and fake news and to verify all claims related to COVID-19 made on social media.  Solution - [cite1, cite2] have taken small steps in this direction.

Owing to the immense importance of patient data matching, significant advances have been achieved in many aspects of the matching process, but the research is limited to heuristic methods where all the attributes of the patient are checked for potential matches based on the logical rules devised. But this approach is tedious, time-consuming and will fail if there are missing data or if the data formats are different. To overcome both these problems, Machine learning methods were incorporated but they demand labeled data which is not possible to obtain or might create a bias due to the training set distribution. So to overcome all these issues and to address the need of the hour we could offer a solution using a combination of probabilistic matching and machine learning. 

\textbf{There are several upcoming methods and ways scientists and researchers are trying to explore and venture into to track and prevent the exponential transmission of the virus.} A few of the notable mentions of the new and upcoming testing practices are  STOPCovid: an initiative by researchers and scientists from MIT to provide the testing facilities at a cheaper cost available to the non-experts outside the laboratories to carry out the tests in their home or private premises. Next, leveraging AI for Testing, where easier ways could be used to detect COVID such as from sounds of cough, breadth, and saliva.  Using these facilities will not only make the process simpler and easier to carry out by also helping the authorities to broaden the scope of testing and inturn help manage the available capital and supplies but expand testing to community-level including mass population testing. 

There have been researches carried out in this direction but they are limited to resource allocation and Vaccine generation. So matching patient data is of significant importance because errors in data matching possess a considerable threat to the delivery of suitable care and patient safety, and can lead to potentially fatal consequences. A major challenge is a lack of common entity identifiers in the databases to be matched. However, such information is often present in low quality. Personal details especially suffer from frequently occurring typographical variations and errors. 

\begin{figure}[!h]
    \includegraphics[width = .95\linewidth]{images/image--001.jpg}
    \centering
    \caption{<ADD CAPTION>: Source: Unesco. DISINFODEMIC: Deciphering COVID-19 disinformation}
    \label{fig:disinformation}
\end{figure}
\begin{figure}[!h]
    \includegraphics[width = .95\linewidth]{images/4steps.pdf}
    \centering
    % \caption{<ADD CAPTION>: Source: Unesco. DISINFODEMIC: Deciphering COVID-19 disinformation}
    \label{fig:4steps}
\end{figure}

